Launcher Attitude Control based on Incremental Nonlinear Dynamic Inversion: A Feasibility Study Towards Fast and Robust Design Approaches

The so-called ``New Space era'' has seen a disruptive change in the business models and manufacturing technologies of launch vehicle companies. However, limited consideration has been given to the benefits that innovation in control theory can bring; not only in terms of increasing the limits of performance but also reducing mission preparation or ``missionisation'' efforts. Moreover, there is a gap between the current state-of-practice that still relies on linear controls and other modern control techniques that could bring relevant improvements in launcher attitude control. Nonlinear Dynamic Inversion (NDI) is a technique that basically `cancels' the nonlinearities of a class of nonlinear systems, allowing for a single linear control law to be applied without the need for gain-scheduling across different operational points. Incremental NDI (INDI) is a variation of NDI that generates incremental commands and employs acceleration feedback to reduce model dependency, making it easier to design, and results in being more robust in closed-loop. While INDI has been applied successfully to several aerospace applications, its applicability to launch vehicles has not yet been adequately investigated. The objective of this paper is therefore to introduce and raise awareness of the INDI method among the launcher guidance, navigation, and control (GNC) community, showcasing its implementation on a representative launch ascent application scenario which highlights INDI's strengths and challenges. We present a new, practical approach for stability analysis of INDI for attitude control, and compare INDI with scheduled PD controllers with- and without angular acceleration estimates. Results show that, while INDI controllers are generally more sensitive to sensor noise and actuator delay than linear controllers, their potential benefits outweigh these limitations in terms of robustness and performance.

==> include/gnc-extended-abstract.tex <==
\begin{center}{\footnotesize\textit{{\color{blue}---Extended abstract, to be reduced---}}}\end{center}

{\footnotesize{
The so-called ``New Space era'' has been marked by a disruptive change in the business models, manufacturing technologies and agile practices of launch vehicle companies, aimed at minimising their production and operating costs in an ever more competitive market. Yet, only limited consideration has been given to the benefits that innovation in the field of control theory can bring, not only in terms of increasing the limits of performance, but also reducing mission preparation (``missionisation'') efforts. Also on government-led developments, recent launchers such as Ares I and VEGA [R1] still use the same design approach of the Saturn V rocket, i.e. linear controllers. This approach relies on single channel-at-a-time tuning and ad hoc gain-scheduling followed by extensive V\&V, which are very time and cost consuming processes.\\

In contrast to the approach presented above, the past few years have seen a growing interest in the application of artificial intelligence and machine learning methods for launcher GNC, but the industrial use of such data-driven/model-free methods remains limited by well-known issues related to training and certification of the algorithms on the full flight envelope of intended operation. In that sense, there is a clear gap between these strategies and the current state-of-practice, in which other techniques could bring relevant improvements; this is the case for nonlinear control algorithms, especially those based on Nonlinear Dynamic Inversion (NDI). On one hand, agile practices of New Space companies provide the ideal opportunity to explore the benefits of this type of design approach. On the other hand, a successful adoption of nonlinear launcher control will likely facilitate the augmentation with and transition to data-driven methods in the future.\\

The NDI technique consists in cancelling the nonlinearities of a nonlinear system by means of state feedback so that the system is transformed into a linear form (for this reason, NDI is often known as “feedback linearisation”). For the resulting linear system, a single linear control law can be applied without the need for gain-scheduling to tailor the controller to different conditions. Being a multivariable technique, NDI allows to decouple and handle all the control channels in a systematic manner. The main drawback of this technique is that the linearisation fully relies on the accurate knowledge of the system, thus model mismatches may lead to substantial performance and stability losses. To tackle this drawback, an approach called Incremental NDI (INDI) was proposed in the early 2000s. By generating incremental commands (instead of total inputs) and employing acceleration feedback, the model dependency of the INDI technique is greatly reduced (for this reason, INDI is also known as a “sensor-based” approach). Being less model-dependent, INDI-based controllers become easier to design and significantly more robust. The resulting nonlinear control law still relies on an approximate model of the system’s control effectiveness, which in turn can be integrated with data-driven methods.\\

Incremental NDI has been elaborated theoretically and applied successfully to high-performance systems including advanced aircraft flight control and a few studies for spacecraft attitude control. More recently, it has been applied to fault-tolerant control of aircraft subjected to sensor and actuator faults, as well as in real flight tests of small unmanned aircraft and of a business passenger jet [R2], demonstrating INDI’s performance and robustness against aerodynamic model uncertainties and disturbance rejection. However, to the best of the authors’ knowledge, its applicability to launch vehicles has never been adequately investigated. The potential benefits of INDI become even more relevant for the case of reusable launchers, which are characterised by much tighter dynamical couplings between (online-generated) trajectory and attitude during descent flight.
It is therefore the objective of this study to present and raise awareness of the INDI technique among the launcher GNC community, to showcase its implementation on a representative application scenario, and to highlight its strengths and challenges in the face of the industrial state-of-practice. To achieve this, the paper provides a concise description of the NDI and INDI approach, followed by the detailed design and comparison of different control laws: linear, linear with angular acceleration feedback and INDI-based. The application scenario is that of a launcher model in ascent flight featuring attitude and drift degrees-of-freedom, actuator dynamics and moving-mass effects. All the controllers and filters are implemented at a sampling frequency that is compatible with current onboard capabilities (25 Hz).\\

There are mainly two well-known challenges associated with the practical implementation of INDI-based control. The first one is that, by relying on angular acceleration and control input measurements/estimates, INDI controllers are generally more sensitive to sensor noise and actuator delay than classical controllers. The second challenge of INDI is that, due to its nonlinear nature, attaining an analytical proof of stability is not trivial [R3]. To assess the severity of the first challenge, the paper shows a comprehensive nonlinear simulation campaign with wind disturbances, uncertainties, as well as different levels of sensor noise and actuator delay. For the second challenge, the paper proposes a simple yet insightful linearisation-based approach to evaluate stability degradation related to an inexact feedback linearisation and to deviations from the control tuning conditions.
From the results obtained in this feasibility study, the two limitations above seem to be outweighed by the potential benefits of INDI-based launcher control. Further analysis on this topic will address the impact of flexible modes and non-collocated sensing.
}}

==> include/gnc-whiteboard.tex <==
NDI consists on the application of the following input
transformation~[{khalil2002, slotine1990, acquatella2020phd}]
\begin{equation}\label{eq:input-transformation-MIMO}
	\ur_{{\text{cmd}}} =
	\gr^{-1}(\xr)\left(\nux - \fr(\xr)\right)
\end{equation}
which
cancels all nonlinearities in closed-loop, 
and a simple linear input-output relationship 
between the new virtual control input 
$\nux$ and the output $\yr$ is obtained
\begin{align}\label{eq:linear-MIMO}
	\dot{\yr} = \nux .
\end{align}

Apart from being linear, an interesting result from this relationship 
is that it is also decoupled since the input $\nu_i$ only affects the 
output $\ys_i$. From this fact, the input transformation 
\eqref{eq:input-transformation-MIMO} is called a \textit{decoupling control law},
and the resulting linear system \eqref{eq:linear-MIMO} is called 
the \textit{single-integrator} form. This single-integrator form 
\eqref{eq:linear-MIMO} can be rendered exponentially stable with
\begin{align}\label{eq:virtual-control-law-error}
	\nux = \dot{\yr}_{\text{des}} = \dot{\yr}_{\text{cmd}} + \Kr_P\,\boldsymbol{e}
\end{align}
where $\dot{\yr}_{\text{des}}$ defines the desired dynamics
for the output vector or control variables, 
$\dot{\yr}_{\text{cmd}}$ is the feedforward term for tracking, 
\mbox{$\boldsymbol{e} = {\yr}_{\text{cmd}} - {\yr}$} is the error vector,
${\yr}_{\text{cmd}}$ denotes the smooth desired 
output vector (at least one time differentiable),
and $\Kr_P\in\reals{m\times m}$ is a diagonal matrix, 
whose $i-$th diagonal elements $K_{P_i}$ 
are chosen so that the polynomials
\begin{align}\label{eq:error-poly}
	s + K_{P_i}, \qquad i = \{1,\ldots,m\}
\end{align}
may become Hurwitz. This results in the exponentially 
stable and decoupled \textit{desired} error dynamics
\begin{align}\label{eq:error-dyn}
	\dot{\boldsymbol{e}} + \Kr_P\,\boldsymbol{e} = \boldsymbol{0},
\end{align}
which implies that $e_i(t)\rightarrow 0,~i=\{1,\ldots,m\}$.	
From this typical tracking problem, and as illustrated in Figure~\ref{fig:sr_ndi}, 
it can be seen that the entire control system will have two control loops~[{acquatella2020phd}]: 
the inner linearization loop based on Equation~\eqref{eq:input-transformation-MIMO},
and the outer control loop in Equation~\eqref{eq:virtual-control-law-error} 
based on linear control.
\begin{figure}[h!]
	\centering
	%	\includegraphics[scale=0.35]{sr/pic/sr_ndi.png}
	\caption{Tracking of a MIMO system with Nonlinear Dynamic Inversion. The inner linearization loop is
		based on Equation~\ref{eq:input-transformation-MIMO}, 
		whereas each channel $y_i − \nu_i$ of the outer control loop is based on a linear control $K(e,\dot{e},\ldots)$. Source~[{acquatella2020phd}].}
	\label{fig:sr_ndi}
\end{figure}

Finding an explicit relationship between the input $u$
and the output $y$ is generally not straightforward
because they are not directly related.
Consider again the generic model of affine 
$n$-dimensional multivariable nonlinear systems 
described in Eqs.~\eqref{eq:nonlinear-mimo-dyn-a}--\eqref{eq:nonlinear-mimo-dyn-b}.
%
Collecting all differentiated outputs $y_i$ results in $m$ equations
in the form of (with a slight abuse of notation using $(\cdot)^{(\rhor)}$)
%
\begin{equation}\label{eq:diff-outputs}
	\yr^{(\rhor)} = \lr(\xr) + \Mr(\xr)\ur
\end{equation}
%
with
%
\begin{equation*}
	\yr^{(\rhor)} =
	\left[
	\begin{array}{c} 
		y_{1}^{(\rho_1)} \\
		y_{2}^{(\rho_2)} \\
		\vdots \\
		y_{m}^{(\rho_m)} \\
	\end{array}
	\right],\,
	\lr(\xr) =
	\left[
	\begin{array}{c} 
		{\mathcal{L}}_{f}^{\rho_1}h_1(\xr) \\
		{\mathcal{L}}_{f}^{\rho_2}h_2(\xr) \\
		\vdots \\
		{\mathcal{L}}_{f}^{\rho_m}h_m(\xr) \\
	\end{array}
	\right],\,
\end{equation*}
\begin{equation*}
	\Mr(\xr) =
	\left[
	\begin{array}{cccc} 
		{\mathcal{L}}_{g_1}{\mathcal{L}}_{f}^{\rho_1-1}h_1(\xr) & 
		{\mathcal{L}}_{g_2}{\mathcal{L}}_{f}^{\rho_1-1}h_1(\xr) & \cdots & 
		{\mathcal{L}}_{g_m}{\mathcal{L}}_{f}^{\rho_1-1}h_1(\xr) \\
		{\mathcal{L}}_{g_1}{\mathcal{L}}_{f}^{\rho_2-1}h_2(\xr) & 
		{\mathcal{L}}_{g_2}{\mathcal{L}}_{f}^{\rho_2-1}h_2(\xr) & \cdots & 
		{\mathcal{L}}_{g_m}{\mathcal{L}}_{f}^{\rho_2-1}h_2(\xr) \\
		\vdots & \vdots &  & \vdots \\
		{\mathcal{L}}_{g_1}{\mathcal{L}}_{f}^{\rho_m-1}h_m(\xr) &
		{\mathcal{L}}_{g_2}{\mathcal{L}}_{f}^{\rho_m-1}h_m(\xr) & \cdots & 
		{\mathcal{L}}_{g_m}{\mathcal{L}}_{f}^{\rho_m-1}h_m(\xr) 
	\end{array}
	\right]
\end{equation*}
%
where ${\mathcal{L}}_{f}^{\rho_j}h_j$,
${\mathcal{L}}_{g_i}{\mathcal{L}}_{f}^{\rho_j-1}h_j$
are the Lie derivatives~\cite{slotine1990,khalil2002} 
of the scalar functions $h_j$ 
with respect to the vector fields $\fr$ and $\gr_i$,
where $j,~i=1, 2, \ldots, m$, respectively. 
%
Moreover, the system is said to have a vector of relative
degree $\rhor = [\,\rho_1 \quad \ldots\quad \rho_p \,]\transpose$ 
at some point $\bar{\xr}\in\reals{n}$ of the state--space when there exists a 
region of interest $\boldsymbol{\mathcal{D}}_0\subset\reals{n}$ around $\bar{\xr}$
such that for all $\xr\in\boldsymbol{\mathcal{D}}_0$, $\boldsymbol{M}(\xr)$ is
nonsingular (i.e., invertible) and $
%
%\begin{equation*}
{\mathcal{L}}_{g_i}{\mathcal{L}}_{f}^{k} h_j(\xr) = 0,\,
0 \leq k \leq \rho_j - 1,\,
1 \leq i,~j \leq m$.
%\end{equation*}
%
In other words, the vector of relative degree represents, 
for each output $y_i$, $i = 1,\ldots,p$,
the number of output differentiations needed for the 
input to appear~\cite{slotine1990,khalil2002}.
Moreover, the vector of relative degree of the 
continuous--time nonlinear system satisfies
%
\begin{equation}
	\rho = \left\|\rhor\right\|_1 
	= \sum_{i=1}^{m}\rho_i \leq n
\end{equation}
%
where $\rho$ is henceforth called the 
total relative degree of the system.
Furthermore, the system is said to have
uniform relative degree when $\rho_1 = \rho_2 = \cdots = \rho_m$.
%
% In this paper, since the output is the MRP vector,
% the continuous--time nonlinear system has uniform
% relative degree $\rho_1 = \rho_2 = \rho_3 = 2$ and therefore
% $\rho = 6 < n = 9$. 
%

Denoting the $m$ outputs $y_j$ and their derivatives
up to the ($\rho_j-1$) order as new states
%
\begin{equation}
	\xir = [\,\xir_1 \quad \ldots\quad \xir_{m} \,]\transpose, \quad
	\xir_i = [\,{\xi}^i_1 \quad \ldots\quad {\xi}^i_{\rho_i} \,]\transpose, \quad
	i = 1,\ldots,m
\end{equation}
%
% inline version
%$\xir = [\,\xir_1 \quad \ldots\quad \xir_{m} \,]\transpose$,
%where 
%$\xir_i = [\,{\xi}^i_1 \quad \ldots\quad {\xi}^i_{\rho_i} \,]\transpose$,
%$i = 1,\ldots,m$,
%
if the total relative degree is
equal to the order of the system ($\rho = n$),
the $\rho$--coordinates ${\xi}_{i}^{j},~j = 1,2,\ldots,m;~i = 1,2,\ldots,\rho_j,$
describe fully the nonlinear behavior of the original system, and moreover,
the system is said to be full--state feedback linearizable.
Otherwise, whenever the total relative degree is
strictly less than the order of the system ($\rho < n$),
a part of the system dynamics would become unobservable
via input--output linearization using the new set of 
the $\rho$--coordinates ${\xi}_{i}^{j}$, and therefore,
these coordinates do not fully describe the original system.
In such case, the input--output linearization decomposes the
dynamics of the nonlinear system into an external part (input--output),
described by the $\rho$--coordinates, and an internal part (unobservable),
described by a new set of ($n-\rho$)--coordinates 
and therefore called the internal dynamics of the system.
%
The unobservable states, usually denoted as 
$\etar = [\,\eta_1 \quad \ldots\quad \eta_{n-\rho} \,]\transpose$,
are defined via smooth functions 
$\phir(\xr) = [\,\phi_1 \quad \ldots\quad \phi_{n-\rho} \,]\transpose$
in the neighborhood $\boldsymbol{\mathcal{D}}_0$ of $\xr$
%, $\forall \xr\in\reals{n}$ 
as
%
\begin{equation}
	\etar = \phir(\xr)
\end{equation}
%
such that ($\forall \xr \in \boldsymbol{\mathcal{D}}_0$)
%
\begin{equation}
	\frac{\partial{\phi_i}}{\partial \xr}\gr_j(x) = 0,
	\quad\text{for } 1\leq i \leq n - \rho,
	\quad\text{for } 1\leq j \leq m
\end{equation}
%
Considering a new 
coordinate--system $\boldsymbol{z}$ defined as
%
\begin{equation}\label{eq:diffeo-z}
	\zr = \Tr(\xr) 
	%=
	%\left[
	%\begin{array}{c} 
	%\boldsymbol{T}_1(\xr) \\
	%\midrule
	%\boldsymbol{T}_2(\xr)
	%\end{array}
	%\right]	
	=
	\left[
	\begin{array}{c} 
		\psir(\xr) \\
		\phir(\xr)
	\end{array}
	\right]	
	=
	\left[
	\begin{array}{c} 
		\xir \\
		\etar
	\end{array}
	\right]
\end{equation}
%
where $\Tr$ represents a diffeomorphism on the 
domain $\mathcal{{D}}_0$, then the original nonlinear 
system can be transformed into the normal form~\cite{isidori1985,slotine1990,khalil2002,wang2019indi} as
%
\begin{subequations}\label{eq:nonlinear-mimo-normal-form}
	\begin{align}
		\dot{\xir} 
		&= 
		\Ar_c\xir + 
		\Br_c\left[\lr(\xr) + \Mr(\xr)\ur\right]
		\Big|_{\xr = \Tr\inv(\zr)}
		\label{eq:nonlinear-mimo-normal-form-a} \\
		\dot{\etar} 
		&= 
		\fr_c(\xir,\etar) =
		{\mathcal{L}}_{f}\phir(\xr)
		\Big|_{\xr = \Tr\inv(\zr)} =
		\frac{\partial\phir(\xr)}{\partial\xr}\fr(\xr)
		\Big|_{\xr = \Tr\inv(\zr)}
		\label{eq:nonlinear-mimo-normal-form-b}\\
		{\yr} 
		&= 
		\Cr_c\xir 
		\label{eq:nonlinear-mimo-normal-form-c}
	\end{align}
\end{subequations}
%
where the triplet $(\Ar_c,\Br_c,\Cr_c)$
is in Brunovsky block canonical form, i.\,e., 
$\Ar_c = \text{diag}\{\Ar^i_o\}$,\,
$\Br_c = \text{diag}\{\Br^i_o\}$,\,
$\Cr_c = \text{diag}\{\Cr^i_o\},\,i=1,\ldots,m$,
where $(\Ar^i_o,\Br^i_o,\Cr^i_o)$
is a canonical form representation of a chain of $\rho_i$ integrators.

%
The transformation $\Tr$ is required to be a diffeomorphism
by the necessity of $\Tr$ being invertible
(at least locally in $\boldsymbol{\mathcal{D}}_0$), i.e., 
$\Tr\inv(\Tr(\xr))=\xr,~\forall\xr\in\boldsymbol{\mathcal{D}}_0$, in order to recover the original state 
vector from the new coordinate $\zr$, together with the necessity of $\Tr$ and its inverse
$\Tr\inv$ to be smooth mappings in $\reals{n}$ 
guaranteeing that the description of the nonlinear
system in the new coordinates is still a smooth one. Since it is 
generally difficult to find a diffeomorphism defined for all $\xr\in\reals{n}$,
the requirement of having a diffeomorphism well defined for all
$\xr\in\boldsymbol{\mathcal{D}}_0\subset\reals{n}$ makes it a local one.
%
Defining the vector
$\varphir(\xr)$ 
and matrix $\varthetar(\xr)$ as
%
\begin{subequations}
	\begin{equation}
		\varphir(\xr) = -\Mr^{-1}(\xr)\lr(\xr)
	\end{equation}
	\begin{equation}	
		\varthetar(\xr) = \Mr^{-1}(\xr) 
	\end{equation}
\end{subequations}
%
and denoting $\nux$ as a virtual control input,
the state feedback control law $\ur$ defined as
%
\begin{align}\label{ur:deco-end}
	\ur &= \varphir(\xr)+\varthetar(\xr)\nux
		 = \Mr^{-1}(\xr) \left[\nux - \lr(\xr)\right]
\end{align}
%
cancels all nonlinearities in closed-loop in absence
of external disturbances and model uncertainties, resulting in the system
%
\begin{subequations}\label{eq:nonlinear-mimo-normal-form-closed}
	\begin{align}
		\dot{\xir} 
		&= 
		\Ar_c\xir + 
		\Br_c\nux 
		\label{eq:nonlinear-mimo-normal-form-closed-a} \\
		\dot{\etar} 
		&= 
		\fr_c(\xir,\etar)
		\label{eq:nonlinear-mimo-normal-form-closed-b} \\
		{\yr} 
		&= \Cr_c\xir 
		\label{eq:nonlinear-mimo-normal-form-closed-c}
	\end{align}
\end{subequations}
%
which is still described in normal form 
and decomposed into an external (input--output) part and
an internal (unobservable) part. This resulting system is now 
driven by the virtual control input
and entirely described in the newly 
defined $\zr$--coordinates 
$(\etar,\xir)$.
%
The equation 
$\dot{\etar} = \fr_c(\bm{0},\etar)$
defines the zero--dynamics of the system which is defined
as the internal dynamics that appear in the system when the 
input and the initial conditions are chosen such that
the output is made or kept identically to zero for all $t \geq 0$.
Furthermore, the system is said to be minimum
phase if the zero--dynamics have an asymptotically stable
equilibrium point in the domain of interest~\cite{khalil2002}.
%The zero dynamics can be characterized in the
%x-coordinates
%
Referring back to the $y_i$ differentiated outputs 
in Eq.~\eqref{eq:diff-outputs}, application of the
control input in~\eqref{ur:deco-end} results in 
$m$ equations
in the form of 
$y_i^{(\rho_i)} = \nu_i,~i=\{1,\ldots,m\}$,
%
or, with a slight abuse of notation, more compactly as
%
\begin{equation}\label{res:lin-end}
	\yr^{(\rhox)} = \lr(\xr) + \Mr(\xr)\ur = \nux
\end{equation}
%
and the sought linear input--output 
relationship between the new input $\nux$ and 
the output $\yr$ is obtained
as long as $\varthetar=\Mr^{-1}(\xr)$ is nonsingular. 
%
Apart from being linear, an interesting result from this relationship 
is that it is also decoupled since the input $\nu_i$ only affects the 
differentiated output $y_i^{(\rho_i)}$. 
From this fact, the input transformation~\eqref{ur:deco-end} 
is called a \textsl{decoupling control law},
and the linear system~\eqref{res:lin-end} 
results in an \textsl{integrator--chain}.
%
The integrator--chain~\eqref{res:lin-end} is sought
to be rendered exponentially stable with the proper design of $\nux$.
%for instance such as
%%
%\begin{equation}\label{res:lin-nu}
%	\nux = -k_0 \yr - k_1 \frac{\dif\yr}{\dif t} - k_2 \frac{\dif^2\yr}{\dif t^2} - \cdots
%	- k_{\rhox - 1} \frac{\dif^{(\rhox - 1)}\yr}{\dif t^{(\rhox - 1)}}
%\end{equation}
%
From this typical control problem it can be seen that the entire 
system will have two control loops~\cite{chu2010a,chu2010b,sieberling2010}: 
the inner linearization loop~\eqref{ur:deco-end},
and the outer control loop provided by the design of $\nux$. 
%~\eqref{res:lin-nu}.	 
This resulting NDI control law depends on accurate knowledge
of the model and its parameters, hence it is 
susceptible to model and parametric uncertainties contained in both 
$\lr(\xr)$ and $\Mr(\xr)$.

%\subsubsection{Spacecraft Attitude Control}

\subsection{{INDI}} 

The concept of incremental nonlinear dynamic inversion (INDI) amounts to the application of NDI 
to a system expressed in an incremental form~[{acquatella2020phd}]. 
This improves the robustness of the closed-loop 
system as compared with conventional NDI since dependency on the accurate 
knowledge of the plant dynamics is reduced.
First, we introduce a \textit{sufficiently small} time--delay $\lambda$ 
and define the following deviation variables
$\dot{\xr}_0:= \dot{\xr}(t-\lambda)$,
$\xr_0:= \xr(t-\lambda)$, and
$\ur_0:= \ur(t-\lambda)$,
%
% \begin{subequations}\label{eq:MIMO-dynamics-incremental-derivatives}
% 	\begin{align}
% 		\dot{\xr}_0		    & := \dot{\xr}(t-\lambda) \\ % = f(\omega_0)+G(\omega_0)\delta_0 
% 		\xr_0 				& := \xr(t-\lambda) \\
% 		\ur_0 				& := \ur(t-\lambda)		
% 	\end{align}
% \end{subequations}
%
which are the $\lambda$--time--delayed signals of the current 
state derivative $\dot{\xr}(t)$, state $\xr(t)$, and control $\ur(t)$,
%acceleration $\dot{\omega}$, rate $\omega$, and control $\delta$, 
respectively.
Moreover, we will denote
$\Delta\dot{\xr} := \dot{\xr}-\dot{\xr}_0$,
$\Delta{\xr} := {\xr}-{\xr}_0$, and
$\Delta\ur := \ur-\ur_0$
%
% \begin{subequations}\label{eq:MIMO-dynamics-incremental-terms}
% 	\begin{align}
% 		\Delta\dot{\xr} & := \dot{\xr}-\dot{\xr}_0 \\
% 		\Delta{\xr} 		& := {\xr}-{\xr}_0 \\
% 		\Delta\ur 			& := \ur-\ur_0
% 	\end{align}
% \end{subequations}
%
%as the incremental acceleration, 
%the incremental rate, and
as the incremental state derivative, 
the incremental state, and
the so--called incremental control input, 
respectively.
%
% \subsubsection*{{\color{blue}Incremental Form}}
To obtain an incremental form of system dynamics, we
consider a first-order Taylor series expansion of $\dot{\xr}(t)$ ([{sieberling2010, simplicio2013}]),
not in the geometric sense, 
but with respect to the newly introduced time--delay $\lambda$ as  
%
\begin{align*}\label{eq:taylor-incremental}
	\dot{\xr}  
	= ~ & \dot{\xr}_0 + 
	\frac{\partial}{\partial\xr}
	\big[\boldsymbol{f}(\xr) + \boldsymbol{g}(\xr)\ur\big] \bigg|_{\substack{\xr=\xr_0 \\ \ur=\ur_0}}
	\Delta\xr 
	+ \boldsymbol{g}(\xr_0)\Delta\ur 
	+ \mathcal{O}(\Delta\xr^2) \\ %\textit{H.O.T} \\
	\cong ~ 
	& \dot{\xr}_0 
	+ \boldsymbol{A}_0(\xr_0)\Delta\xr 
	+ \boldsymbol{g}\Delta\ur		
\end{align*}
%
with
%
\begin{subequations}
	\begin{align}
		\dot{\xr}_0 := \dot{\xr}(t-\lambda) 
		= \boldsymbol{f}(\xr_0) + \boldsymbol{g}(\xr_0)\ur_0
	\end{align}
\end{subequations}
%
and
%
\begin{subequations}
	\begin{align}
		\boldsymbol{A}_0(\xr_0) & = \frac{\partial}{\partial\xr}
		\Big[\boldsymbol{f}(\xr) + \boldsymbol{g}(\xr)\ur\Big] 
		\Big|_{\substack{\xr=\xr_0 \\ \ur=\ur_0}} 
		% 		\Mr_0 & = \boldsymbol{M}_0(\xr_0)
	\end{align}
\end{subequations}
%
which represents the Jacobian linearization of the on-board model.
We will refer to $\boldsymbol{g}(\xr_0)$ as the \textit{instantaneous control effectiveness (ICE)} matrix; meaning that this model--based term is sampled at each incremental instant~[{acquatella2020phd}].
This means an approximate linearization about the $\lambda-$delayed signals is performed \textit{incrementally}, and not with respect to a particular equilibrium or operational point of interest.

\noindent\textbf{\textit{Time-scale separation (TSS) assumption:}}
%
\textit{For a sufficiently small time-delay $\lambda$ and for any incremental 
	control input, it is assumed 
	that $\Delta{\xr}$ does not vary significantly during $\lambda$. 
	In other words, the input rate of change
	is much faster than the state rate of change:}
%
\begin{equation}\label{eq:eps-indi-tss}
	{\epsilon_{INDI_{\text{TSS}}}}(t) 
	\equiv \Delta{\xr} := {\xr}-{\xr}_0 \cong 0, ~\forall~\Delta\ur
\end{equation}
%
\textit{which leads to}
%
\begin{align*}\label{eq:taylor-incremental}
	\dot{\xr}
	\cong ~ & 
	\dot{\xr}_0 
	+ \boldsymbol{A}_0\underbrace{\left(\xr-\xr_0\right)}_{\cong 0} + \boldsymbol{g}(\xr_0)\cdot\left(\ur-\ur_0\right)
\end{align*}
%
\textit{or simply}
%
\begin{equation}\label{eq:inc-odot-rep}
	\Delta\dot{\xr} \cong \boldsymbol{g}(\xr_0)\cdot\Delta\ur
\end{equation}
%
This assumption shows that for high sampling rates
the nonlinear system dynamics in its incremental form
is simply approximated by its ICE matrix $\boldsymbol{g}(\xr_0)$. Since this results in a change of coordinates, the development of control laws in the original set of (absolute) coordinates
implies or requires the availability of $\dot{\xr}_0$
and $\ur_0$ in~\eqref{eq:inc-odot-rep}.
%
For the obtained approximation
$\Delta\dot{\xr} \cong \boldsymbol{g}(\xr_0)\cdot\Delta\ur$,
% $\dot{\boldsymbol{\zeta}} \cong \dot{\boldsymbol{\zeta}}_0 + \Mr_0\left(\ur-\ur_0\right)$, 
NDI is applied to obtain a relation between 
the incremental control input and the output of the system
%
\begin{equation}\label{eq:incremental-second-relation}
	\ur = \ur_0 + \boldsymbol{g}(\xr_0)^{-1}(\nux-\dot{\xr}_0)	.
\end{equation}
%
Note that the incremental input $\ur_0$ that corresponds to $\dot{\xr}_0$ 
is obtained from the output of the actuators, and it has been assumed that a 
commanded control is achieved \textit{sufficiently fast} in regards to
the actuator dynamics. The total control command along with the obtained 
linearizing control $\Delta\ur=\ur(t-\lambda)$ can be rewritten as
%
\begin{equation}\label{eq:incremental-final}
	\ur(t) = \ur(t-\lambda) + \Mr(\xr_0)^{-1}[\,\nux-\dot{\xr}(t-\lambda)].
\end{equation}
%
The dependency of the closed-loop system on accurate knowledge of the dynamic model in 
$\boldsymbol{f}(\xr)$ is largely decreased, improving robustness against model uncertainties 
contained therein. Therefore, this implicit control law design is more dependent 
on accurate measurements or accurate estimates of $\dot{\xr}_0$, 
the state derivatives, and $\ur_0$, the incremental control input, respectively. 

Regarding INDI as illustrated in Figure~\ref{fig:sr_indi}, 
it can be seen that the control system will still have two control loops~[{acquatella2020phd}]: 
the inner linearization loop based on Equation~\eqref{eq:incremental-final},
and the outer control loop which is still based on linear control.
%
\begin{figure}[h!]
	\centering
	%	\includegraphics[scale=0.45]{sr/pic/sr_indi.png}
	\caption{Tracking of a MIMO system with Incremental 
		Nonlinear Dynamic Inversion. The inner linearization loop is
		based on Equation~\ref{eq:incremental-final}, 
		whereas each channel $y_i − \nu_i$ of the outer control loop is based on a linear control $K(e,\dot{e},\ldots)$. Source~{acquatella2020phd}.}
	\label{fig:sr_indi}
\end{figure}


\section{NDI Control}

%
The attitude control design begins by first
considering the new coordinate--system given by
the local diffeomorphism~\eqref{eq:diffeo-z} 
%
where the external states
$\boldsymbol{\xi} = [\,\boldsymbol{\xi}_1\quad\boldsymbol{\xi}_2\quad\boldsymbol{\xi}_3\,]\transpose$
are given by
$\boldsymbol{\xi}_i = [\,{\xi}_{i}^{1}\quad{\xi}_{i}^{2}\,]\transpose = 
[\,q_i\quad\dot{q}_i\,]\transpose,~i = 1, 2, 3$,
%
and the choice for the remaining internal state
$\boldsymbol{\eta} = \boldsymbol{\phi}(\xr) = \phi$
is written in compact form as
$\boldsymbol{\phi}(\xr) = \boldsymbol{H}_{\phi}\,\,\xr$
%
and furthermore, the choice of $\boldsymbol{H}_{\phi}$ has been found such that
the following condition
%
\begin{equation}
	\boldsymbol{\phi}(\boldsymbol{0}) = \boldsymbol{0},\quad
	\frac{\partial\boldsymbol{\phi}}{\partial \xr}\gr(\xr)
	= \boldsymbol{0},
\end{equation}
%
is fulfilled according to the definition of $\boldsymbol{\phi}(\xr)$.
%
Then the original nonlinear 
system can be transformed into the 
normal form~\eqref{eq:nonlinear-mimo-normal-form}
and the state feedback
nonlinear dynamic inversion (NDI) control law 
$\ur$ is obtained as in~\eqref{ur:deco-end}
%
\begin{align}
	\ur &= \left[\lr(\xr)\cdot\Gr\right]^{-1}\left[\nux - \lr(\xr) + \Rr^{(\rhox)} \right]
\end{align}
%
while denoting $\nux$ as a virtual control input to be considered later.
%
With this NDI control law, and in absence of external perturbations and model uncertainties, 
the nonlinearity is cancelled resulting in the nominal closed-loop system as
%
\begin{subequations}\label{eq:nonlinear-mimo-normal-form-closed-acs}
	\begin{align}
		\dot{\boldsymbol{\xi}}_{[6]} &= 
		\boldsymbol{A}_{c{[6\times 6]}}\boldsymbol{\xi}_{[6]} + 
		\boldsymbol{B}_{c{[6\times 3]}}\nux_{[3]} \\
		\dot{\boldsymbol{\eta}}_{[3]} &= 
		\boldsymbol{f}_c(\boldsymbol{\xi}_{[6]},\boldsymbol{\eta}_{[3]}) \\	
		{\yr}_{[3]} &= 
		\boldsymbol{C}_{c{[3\times 6]}}\boldsymbol{\xi}_{[6]} 
	\end{align}
\end{subequations}
%
where the subscript indexes indicate the dimensions of the vectors and
matrices, and 
$\boldsymbol{A}_c$, $\boldsymbol{B}_c$, $\boldsymbol{C}_c$ 
are in Brunovsky block canonical form as in Eqs.~\eqref{eq:cont-ss}.
Furthermore, the internal dynamics characterized in the $\xr$-coordinates
are given by
%
\begin{align}
	\boldsymbol{f}_c(\boldsymbol{\xi},\boldsymbol{\eta})
	\Big|_{\xr = \boldsymbol{T}\inv(\boldsymbol{z})} = 
	%\boldsymbol{f}_c(\xr)	=
	\Gr_{12}\inv\dot{\omegax} -\Gr_{13}\inv\dot{\Omegax}_w
\end{align}
%
% 
%\begin{align*}
%\boldsymbol{A}_c
%&= 
%\left[
%\begin{array}{cccccc} 
%0 & 1 & 0 & 0 & 0 & 0 \\
%0 & 0 & 0 & 0 & 0 & 0 \\
%0 & 0 & 0 & 1 & 0 & 0 \\
%0 & 0 & 0 & 0 & 0 & 0 \\
%0 & 0 & 0 & 0 & 0 & 1 \\
%0 & 0 & 0 & 0 & 0 & 0 \\
%\end{array}
%\right],
%\quad
%\boldsymbol{B}_c
%=
%\left[
%\begin{array}{ccc} 
%0 & 0 & 0 \\
%1 & 0 & 0 \\
%0 & 0 & 0 \\
%0 & 1 & 0 \\
%0 & 0 & 0 \\
%0 & 0 & 1
%\end{array}
%\right],
%\quad
%\boldsymbol{C}_c
%= 
%\left[
%\begin{array}{cccccc} 
%1 & 0 & 0 & 0 & 0 & 0 \\
%0 & 0 & 1 & 0 & 0 & 0 \\
%0 & 0 & 0 & 0 & 1 & 0 
%\end{array}
%\right]
%\end{align*}
%
where
the zero--dynamics are be given by
$\boldsymbol{f}_c(\boldsymbol{0},\boldsymbol{\eta}) = \boldsymbol{0}$
%
%\begin{equation}
%	\boldsymbol{f}_c(\boldsymbol{0},\boldsymbol{\eta}) = \boldsymbol{0}
%\end{equation}
%
which makes the system marginally stable at the origin and around
the small neighborhood $\boldsymbol{\mathcal{D}}_0$ in consideration, 
and therefore the spacecraft attitude control system 
is non-minimum phase.
Zero--dynamics defines the internal dynamics 
of the system when the input and the initial 
conditions are chosen such that the output is maintained 
identically to zero at all times. Therefore, whenever 
$\boldsymbol{\xi} = \boldsymbol{0}$ (which implies $\omegax = \boldsymbol{0}$)
we obtain from definition that $\dot{\omegax}=\boldsymbol{0}$ and
$\dot{\Omegax}_w=\boldsymbol{0}$. Note 
that nothing is said about the corresponding ${\Omegax}_w$ which shall remain constant 
and therefore responsible to keep the angular momentum fixed inertially.
%
Furthermore, 
since $\left[\boldsymbol{l}(\xr)\cdot\Gr\right]$ is not singular,
the linear input--output 
relationship between $\ddot{\sigmax}$ and $\nux$ 
is obtained as a double--integrator
%
%
\begin{equation}\label{eq:double-integrator}
	\ddot{\sigmax} =
	\left[
	\begin{array}{c} 
		\ddot{\sigma}_{1} \\
		\ddot{\sigma}_{2} \\
		\ddot{\sigma}_{3}
	\end{array}
	\right]	
	=
	\left[
	\begin{array}{c} 
		\nu_x \\
		\nu_y \\
		\nu_z
	\end{array}
	\right]
	= \nux
\end{equation}
%
We denote $\er = \sigmax_{e} = \sigmax_{d} - \sigmax$, which is a valid
representation of the MRP error for small rotations~\cite{mrp2008}, and therefore
$\dot{\er} = \dot{\sigmax}_{e} = \dot{\sigmax}_{d} - \dot{\sigmax}$.
The double-integrator~\eqref{eq:double-integrator} can be therefore 
rendered exponentially stable with
%
\begin{align}\label{eq:nux}
	\nux = \ddot{\sigmax}_{d} + \ks_D\dot{\er} + \ks_P\er 
\end{align}
% 
where $\ddot{\sigmax}_{d}$ is the feedforward reference term for tracking tasks, and
$\ks_D$ and $\ks_P$ being $3\times 3$ constant diagonal matrices whose $i-$th
diagonal elements $\ks_{D_i}$ and $\ks_{P_i}$, respectively, 
are chosen so that the polynomials $s^2 + \ks_{D_i}s + \ks_{P_i} ~ i = 1, \ldots , n = 3,$
%
%\begin{align}\label{eq:virtual-control-law-error-hur}
%	s^2 + \ks_{D_i}s + \ks_{P_i} ~ i = 1, \ldots , n = 3
%\end{align}
%
may become Hurtwiz. This results in the exponentially stable and decoupled error dynamics $\ddot{\er} + \ks_D\dot{\er} + \ks_P\er = \zero$
%
%\begin{align}\label{eq:virtual-control-law-error}
%	\ddot{\er} + \ks_D\dot{\er} + \ks_P\er = \zero
%\end{align}
% 
which implies that $\er(t)\rightarrow\zero$ as $t\rightarrow\infty$.

